Masked Linear Regression for Learning Local Receptive Fields for Facial Expression Synthesis

Compared to facial expression recognition, expression synthesis requires a very high-dimensional mapping. This problem exacerbates with increasing image sizes and limits existing expression synthesis approaches to relatively small images. We observe that facial expressions often constitute sparsely distributed and locally correlated changes from one expression to another. By exploiting this observation, the number of parameters in an expression synthesis model can be significantly reduced. Therefore, we propose a constrained version of ridge regression that exploits the local and sparse structure of facial expressions. We consider this model as masked regression for learning local receptive fields. In contrast to the existing approaches, our proposed model can be efficiently trained on larger image sizes. Experiments using three publicly available datasets demonstrate that our model is significantly better than $\ell_0, \ell_1$ and $\ell_2$-regression, SVD based approaches, and kernelized regression in terms of mean-squared-error, visual quality as well as computational and spatial complexities. The reduction in the number of parameters allows our method to generalize better even after training on smaller datasets. The proposed algorithm is also compared with state-of-the-art GANs including Pix2Pix, CycleGAN, StarGAN and GANimation. These GANs produce photo-realistic results as long as the testing and the training distributions are similar. In contrast, our results demonstrate significant generalization of the proposed algorithm over out-of-dataset human photographs, pencil sketches and even animal faces.

==> GAN.tex <==
The most recent advances in expression synthesis have been achieved via 
Generative Adversarial Networks (GANs). A typical GAN consists of two competing 
networks:  a generator that takes a random noise vector (and conditioning 
input) and generates a fake image, and  a discriminator network that 
predicts the probability of an input image being real or fake. These two 
networks compete against each other to update their weights via minimax 
learning. Conditional GANs (cGANs) condition their generator and discriminator 
with additional information such as images or labels. Recently, GAN based 
frameworks have shown impressive results in image-to-image translation tasks. 
Pix2pix \citep{pix2pix2016} is a paired image-to-image translation framework 
based on cGAN and $\ell_1$ reconstruction loss. Unpaired image-to-image 
translation has also been successfully demonstrated by \citep{CycleGAN2017, 
DiscoGAN2017, liu-2017, yi2017dualgan}. CycleGAN \citep{CycleGAN2017} learns a 
mapping between two different domains and incorporates a cycle-consistency loss 
with an adversarial loss to preserve key attributes between the two domains. 
\cite{liu-2017} have proposed  UNIT framework that combines  variational 
autoencoder with  Coupled GAN \citep{liu2016coupled}. UNIT consists of two 
generators that share the latent space between two different domains.  
All of the above-mentioned approaches are designed for translations between two 
domains at a time. More recently, multi-domain image-to-image translation 
frameworks have also been proposed. StarGAN \citep{StarGAN2018} learns mappings among 
multiple domains using a single generator conditioned on the target domain 
labels. The GANimation model of \cite{pumarola_ijcv2019} introduced a framework that takes continuous target domain labels in the form of action units and can produce varying degrees of expressions containing multiple action units. Their method is more accurately described as an expression transfer method instead of synthesis. Their method translates a source face via automatically detected action units from a target face. Reliable automatic extraction of action units from face images is a prerequisite for their method to work properly. 

Most of these GAN based frameworks share the 
same problem with other generative models, that is, partial control over the generated images. These methods synthesize the whole image, and  therefore 
also influence attributes in addition to those that were targeted. Strict local 
control over generated faces is not guaranteed, though some recent GANs 
have attempted that as well \citep{shen2017-ResGAN, zhang2018-saGAN}. Image to image translation using GANs being a very recent research direction, has been quickly progressing. 


In the current work we compare the performance of four GANs including Pix2Pix, CycleGAN, StarGAN and GANimation with the proposed Masked Regression (MR) algorithm. These GANs produce excellent results if the test image has similar distribution as the training dataset. As the distribution of test image diverges from the training dataset distribution, the performance of these GANs deteriorates. In contrast to these GANs, the proposed MR algorithm generalises well to very different type of images, can be trained using very small datasets, have a closed form solution with very small spatial as well as computational complexity. To the best of our knowledge, no such technique has been proposed before us for facial expression synthesis.

